Electrochemical Communication in Bacterial Biofilms: A Study on Potassium Stimulation and Signal Transmission

Electrochemical communication is a mechanism that enables intercellular interaction among bacteria within communities. Bacteria achieves synchronization and coordinates collective actions at the population level through the utilization of electrochemical signals. In this work, we investigate the response of bacterial biofilms to artificial potassium concentration stimulation. We introduce signal inputs at a specific location within the biofilm and observe their transmission to other regions, facilitated by intermediary cells that amplify and relay the signal. We analyze the output signals when biofilm regions are subjected to different input signal types and explore their impact on biofilm growth. Furthermore, we investigate how the temporal gap between input pulses influences output signal characteristics, demonstrating that an appropriate gap yields distinct and well-defined output signals. Our research sheds light on the potential of bacterial biofilms as communication nodes in electrochemical communication networks.

==> system_model.tex <==
\section{One-dimensional Model}

\subsection{Exterior Glutamate and Potassium Concentration}

The following equations describe the dynamics of exterior glutamate and potassium concentrations, denoted by $G$ and $K$, respectively:

\begin{align}
\frac{\partial G}{\partial t} = & D_{G} \frac{\partial^{2} G}{\partial x^{2}} - \frac{\delta_{G}}{\left(1+\exp\left(V-V_{\text{thresh}}\right)\right)} G\left(G_{\max}-G_{\text{intr}}\right),\label{eq:G_ex} \\
\frac{\partial K}{\partial t} = & D_{K} \frac{\partial^{2} K}{\partial x^{2}} + F g_{K} n^{4}\left(V-V_{K}\right) + F g_{L}\left(V-V_{L}\right) - \max\left(\gamma_{K} K\left(K_{\max}-K_{\text{intr}}\right), 0\right) \label{eq:K_ex}.
\end{align}

In these equations, the first terms represent the diffusion of glutamate and potassium through the exterior of the cells within the biofilm, with $D_G$ and $D_K$ being the diffusion coefficients for glutamate and potassium, respectively.

The glutamate uptake by the cell is modulated by the membrane potential $V$ of the cell. This uptake is reduced when the membrane potential $V$ is close to the homeostatic voltage potential $V_{\text{thresh}}$. The glutamate uptake also depends on the glutamate availability at the exterior of the cell and the cell's need for glutamate, which is represented by the difference between the maximum interior glutamate concentration $G_{\max}$ and the actual interior glutamate concentration $G_{\text{intr}}$. These factors are taken into account in the second term of Equation \eqref{eq:G_ex}.

The movement of potassium ions occurs through potassium gates and leak gates. The potassium and leak gates are controlled by the gating parameter $n$ and the reversal potentials of potassium and leak gates $V_K$ and $V_L$, respectively. The uptake and release of potassium through these channels are modeled using the Hodgkin-Huxley model, and they are described by the second and third terms of Equation \eqref{eq:K_ex}. The last term in Equation \eqref{eq:K_ex} represents the potassium pump that transports potassium ions from the exterior to the interior of the cell. The pump takes up potassium if the internal concentration $K_{\text{intr}}$ is below a certain threshold represented by $K_{\max}$.
\subsection{Boundary Conditions}

The boundary conditions for glutamate and potassium at the biofilm boundary are given by Neumann flux conditions, as follows:

\begin{align}
D_{G} \frac{\partial G}{\partial x} = \frac{D_{G}^{fl}}{B_{L}} \left(G_{0} - G_{\text{intrf}}\right), \\
D_{K} \frac{\partial K}{\partial x} = \frac{D_{K}^{fl}}{B_{L}} \left(K_{0} - K_{\text{intrf}}\right),
\end{align}

Here, $D_{G}^{fl}$ and $D_{K}^{fl}$ are the diffusion rates of glutamate and potassium in the fluid, respectively. $G_{0}$ and $K_{0}$ are the long-range concentrations of glutamate and potassium, and $G_{\text{intrf}}$ and $K_{\text{intrf}}$ are the interfacial concentrations of glutamate and potassium, respectively. The parameter $B_{L}$ represents the boundary layer width.

It is important to note that at the boundary $x=0$, we have $\frac{\partial G}{\partial x} = 0$ and $\frac{\partial K}{\partial x} = 0$. This means that there is no net flux of glutamate and potassium at the biofilm's edge, indicating that the transport of these substances is balanced at the boundary.
\subsection{Interior Glutamate and Potassium Concentration}

The dynamics of interior glutamate and potassium concentrations within the bacterial cell are given by the following equations:

\begin{align}
\frac{d G_{\text{intr}}}{d t} = & \frac{\delta_{G}}{\left(1+\exp\left(V-V_{\text{th}}\right)\right)} G\left(G_{\text{max}}-G_{\text{intr}}\right) - \gamma_{G} G_{\text{intr}}\left(M_{\text{grow}} + r_{b}\right) - \frac{\partial}{\partial x}\left(U G_{\text{intr}}\right), \label{eq:G_int} \\
\frac{d K_{\text{intr}}}{d t} = & -F g_{K} n^{4}\left(V-V_{K}\right) - F g_{L}\left(V-V_{L}\right) + \max\left(\gamma_{K} K\left(K_{\text{max}}-K_{\text{intr}}\right), 0\right) \nonumber\\
& - \frac{\partial}{\partial x}\left(U K_{\text{intr}}\right), \label{eq:K_int}
\end{align}

In these equations, $\gamma_G$ represents the glutamate consumption rate, $r_b$ represents the glutamate utilized for metabolic activities, and $M_{\text{grow}}$ represents the growth propensity of the bacterial cell. The parameter $U$ represents the biofilm growth velocity. When the bacteria are under stress, $M_{\text{grow}}$ becomes small, reducing the cells' glutamate consumption. The value of $M_{\text{grow}}$ is given by the expression:

\begin{align}
M_{\text{grow}} = \frac{T_G}{T_G + T_V},
\end{align}

where 
$$T_G = \frac{\frac{G_{\text{intr}}}{G_{\max}}+0.9}{\frac{G_{\text{intr}}}{G_{\max}}+0.9}$$
is a Hill function that becomes large when $G_{\text{intr}}$ is larger than the lower bound $G_u$, and $T_V = \eta_{V} \tanh\left(\gamma_{V}\left(V / V_{\text{low}} - 1\right)\right) + 1$ is a hyperbolic tangent activation function that becomes large when the membrane potential $V$ is above the bound $V_{\text{low}}$. Parameters $\eta_V$ and $\gamma_V$ are shape parameters.

The growth velocity ($U$) and the growth of the biofilm's length ($L$) are defined as follows:

\begin{align}
U(x) & = \delta_{\text{grow}} \int_{0}^{x} G_{\text{intr}} M_{\text{grow}} dx, \\
\frac{d L}{d t} & = \delta_{\text{grow}} \int_{0}^{L} G_{\text{intr}} M_{\text{grow}} dx,
\end{align}

where $\delta_{\text{grow}}$ is the growth rate.

Bacteria can acclimatize to a range of potassium levels over time, making changes in potassium a better indicator of cellular stress. Let $K_{\text{acclimated}}$ represent the potassium level to which the cells are accustomed. Then, its dynamics are governed by the equation:

\begin{align}
\frac{d K_{\text{acclimated}}}{d t} = \eta_{K}\left(K-K_{\text{acclimated}}\right) - \frac{\partial}{\partial x}\left(U K_{\text{acclimated}}\right),
\end{align}

$K_{\text{acclimated}}$ also affects the reverse potential of the leakage gate.

\subsection{Set of Equations Governing Voltage Potential}

The set of equations representing the voltage potential within the biofilm is given by:

\begin{align}
\frac{d V}{d t} = & -g_{k} n^{4}\left(V-V_{K}\right)-g_{L}\left(V-V_{L}\right) + \max\left(\gamma_{K} K\left(K_{\max }-K_{\text{in}}\right), 0\right) / F - \frac{\partial}{\partial x}(U V), \\
\frac{d n}{d t} = & \alpha \frac{\left(G_{\max }-G_{\text{in}}\right)^{m}}{\left(G_{\max }-G_{l}\right)^{m}+\left(G_{\max }-G_{\text{in}}\right)^{m}}(1-n) - \beta n - \frac{\partial}{\partial x}(U n), \\
V_{K} = & V_{K0} + \delta_{K} K, \\
V_{L} = & V_{L0} + \delta_{L}\left(K-K_{\text{acclimated}}\right),
\end{align}

where $V$ is the voltage potential, $n$ is the gating parameter, $g_k$ and $g_L$ are the conductances for potassium and leak channels, respectively. The term $\max\left(\gamma_{K} K\left(K_{\max }-K_{\text{in}}\right), 0\right) / F$ represents the contribution of potassium dynamics to the voltage potential. The parameter $U$ represents the biofilm growth velocity, and its effect on voltage potential is included through the term $\frac{\partial}{\partial x}(U V)$.

The dynamics of the gating parameter $n$ are described by an equation involving $\alpha$, $\beta$, $m$, $G_{\max}$, $G_{l}$, and $G_{\text{in}}$ (the interior glutamate concentration).

The initial conditions for the simulations are as follows: $G=30\text{ mM}$, $K=8\text{ mM}$, $K_{\text{intr}}=300\text{ mM}$, $K_{\text{acclimated}}=8\text{ mM}$, $V=-160\text{ mV}$, and $n=0.1$. These initial conditions represent the starting state of the biofilm before the simulation begins.
\begin{table}[ht]
    \centering
    \begin{tabular}{c|c|c}
       Name  & Description & Value \\
       $D_G$  &Glutamate diffusion coefficient in biofilm &$0.540 mm^2/day$\\
       $D_K$& Potassium diffusion coefficient in biofilm & $0.497 mm^2/day$\\
$D_G^{f l}$ &  Glutamate diffusion coefficient in fluid  & $0.900 \frac{\mathrm{mm}^2}{\text { day }}$ \\
$D_K^{f l}$ & Potassium diffusion coefficient in fluid  & $4.97 \frac{\mathrm{mm}^2}{\text { day }}$ \\
$G_0$ & Glutamate concentration at inlet  & 30 $\mathrm{mM}$ \\
$K_0$ & Potassium concentration at inlet  & 8 $\mathrm{mM}$ \\
$\delta_G$ & Glutamate uptake rate  & $10 \frac{1}{hour}$ \\
$V_{\thresh}$ & Voltage above which cells cannot uptake glutamate  & $-150 \mathrm{mV}$ \\
$G_{\max} $&  Maximum glutamate concentration in cell  & $20 \mathrm{mM}$ \\
$F$ & Voltage to potassium conversion factor  & $5.6 \frac{\mathrm{mM} \mathrm{K}}{\mathrm{mV}} $\\
$g_K$ &  Potassium gate strength  &$ 180 / \text { hour }$ \\
$g_L$ & Leak gate strength  & $1.2 / \mathrm{hour}$ \\
$\gamma_K$ &  Potassium pump strength  & $.025 / (\text { hour } \times \mathrm{mM} \mathrm{K}) $\\
$B_L$ &  Boundary layer length  & $0.5 \mathrm{~mm}$ \\
$\gamma_G$ & Glutamate consumption rate  & $1.125 / \text { hour }$\\
$r_b$ &  Glutamate basal consumptions rate  & $ 0.1 \text { (dimensionless)}$  \\
$G_u$ & Glutamate bound below which the cells do not grow  & $18 \mathrm{mM} \text { Glutamate }$\\
$\eta_V$ &  Voltage influence in  $M_{\text {grow }}$ & 20 \text { (dimensionless) } \\
$\gamma_V$ &  Voltage transition speed in  $M_{\text {grow }}$ & 20 \text { (dimensionless) } \\
$V_{\text {low }}$ &  Voltage below which cells do not grow  & $-175 \mathrm{mV}$ \\
$\delta_{\text {grow }} $&  Biomass produced in growth  & $\frac{0.0075 mm}{ mM \ Glutamate \times hour}$ \\
$\eta_K$ &  Cells' acclimation rate to potassium change  & 30/ \text{$ hour $} \\
$\alpha$ & Potassium gate opening rate  & $5 / \text { hour }$ \\
$\beta $&  Potassium gate closing rate  & $2.5 / \text { hour }$ \\
$m $&  Potassium gate exponent  & $2 \text { (dimensionless) }$ \\
$G_l$ &  Glutamate level below which cells hyperpolarize  & $10 \mathrm{mM} \text { Glutamate }$ \\
$V_{K 0} $&  Basal potassium gate reversal potential  & $-380 \mathrm{mV}$ \\
$V_{L 0}$ &  Basal leak gate reversal potential  &  $-156 \mathrm{mV}$\\
$\delta_K$ &  Potassium gate reversal change  & $1 \frac{\mathrm{mV}}{\mathrm{mM}} $ \\
$\delta_L$ &  Leak gate reversal change  & $60 \frac{\mathrm{mV}}{\mathrm{mM}} $
    \end{tabular}
    \caption{Parameters for simulation}
    \label{tab:my_label}
\end{table}
